Electroweak corrections to WWZ and ZZZ production at the linear collider

We calculate the electroweak corrections to the production of WWZ and ZZZ at the linear collider in the Standard Model. These processes are important for the extraction of the quartic couplings of the massive gauge bosons which can be a window on the mechanism of spontaneous symmetry breaking. We find that the weak corrections to some kinematic distributions show new features and hence cannot be explained by an overall scale factor.

==> Makefile <==
# Makefile for generating presentation $(TARGET).pdf from $(TARGET).tex

TARGET = main
Subfiles = main.tex

PLOTS = psfig/rs_born_nlo_MH120_ZZZ.eps \
psfig/yW+_born_nlo_MH120_WWZ.eps \
psfig/yW+_delta_nlo_MH120_WWZ.eps \
psfig/pTW_born_nlo_MH120_WWZ.eps \
psfig/pTW_delta_nlo_MH120_WWZ.eps \
psfig/rs_born_nlo_MH120_WWZ.eps

all: $(TARGET).ps $(Subfiles)

tgz: $(Subfiles) $(PLOTS) Makefile
	tar cvzf paper.tar.gz $^

$(TARGET).ps: $(TARGET).tex $(Subfiles)
#	latex $(TARGET).tex
#	bibtex $(TARGET)
	latex $(TARGET).tex
	latex $(TARGET).tex
	dvips $(TARGET).dvi -o
	ps2pdf $(TARGET).ps $(TARGET).pdf
#	xpdf $(TARGET).pdf &

clean:
	rm -f *.dvi *.log *.aux *~ main.ps main.pdf *.blg paper.tgz


